Fisher Flow Matching for Generative Modeling over Discrete Data

Generative modeling over discrete data has recently seen numerous success stories, with applications spanning language modeling, biological sequence design, and graph-structured molecular data. The predominant generative modeling paradigm for discrete data is still autoregressive, with more recent alternatives based on diffusion or flow-matching falling short of their impressive performance in continuous data settings, such as image or video generation. In this work, we introduce Fisher-Flow, a novel flow-matching model for discrete data. Fisher-Flow takes a manifestly geometric perspective by considering categorical distributions over discrete data as points residing on a statistical manifold equipped with its natural Riemannian metric: the $\textit{Fisher-Rao metric}$. As a result, we demonstrate discrete data itself can be continuously reparameterised to points on the positive orthant of the $d$-hypersphere $\mathbb{S}^d_+$, which allows us to define flows that map any source distribution to target in a principled manner by transporting mass along (closed-form) geodesics of $\mathbb{S}^d_+$. Furthermore, the learned flows in Fisher-Flow can be further bootstrapped by leveraging Riemannian optimal transport leading to improved training dynamics. We prove that the gradient flow induced by Fisher-Flow is optimal in reducing the forward KL divergence. We evaluate Fisher-Flow on an array of synthetic and diverse real-world benchmarks, including designing DNA Promoter, and DNA Enhancer sequences. Empirically, we find that Fisher-Flow improves over prior diffusion and flow-matching models on these benchmarks.

==> figures/simplex_geometry.tex <==
\tdplotsetmaincoords{70}{110}
$
\begin{gathered}
\begin{tikzpicture}[tdplot_main_coords, inner sep = 0pt]
\def\laxis{4}
\def\ltriangle{3}
\def\ltick{.2}
%%% axes
%\draw [->] (0,0,0) -- (\laxis,0,0) node [below] {};
%\draw [->] (0,0,0) -- (0,\laxis,0) node [right] {};
%\draw [->] (0,0,0) -- (0,0,\laxis) node [left] {};
%%% axes ticks
\pgfmathtruncatemacro{\nticks}{floor(\laxis)-1}
%%% figure
\filldraw [opacity=.33,blue!60!cyan] (\ltriangle,0,0) -- (0,\ltriangle,0)
-- (0,0,\ltriangle) -- cycle;
\node (pointA) at (0, \ltriangle, 0) {};
\node (pointB) at (0,0,\ltriangle) {};
\node (pointC) at (\ltriangle,0,0) {};
\node (centre) at (\ltriangle / 3, \ltriangle / 3, \ltriangle / 3) {};
\draw[-, thick] (centre) -- (pointA);
\draw[-, thick] (centre) -- (pointB);
\draw[-, thick] (centre) -- (pointC);
\filldraw[black] (pointA) circle (2pt);
\filldraw[black] (pointB) circle (2pt);
\filldraw[black] (pointC) circle (2pt);
\filldraw[black] (centre) circle (2pt);
\end{tikzpicture}
\end{gathered}
\begin{tikzpicture}
\draw[->, ultra thick, bend left=0.5cm] (0, 0) to (2, 0);
\draw[->, ultra thick, bend left=0.5cm] (2, -1) to (0, -1);
\end{tikzpicture}
\begin{gathered}
\begin{tikzpicture}[tdplot_main_coords, inner sep = 0pt]
\def\laxis{4}
  \def\ltriangle{3}
  \def\ltick{.2}
  %%% axes
  %\draw [->] (0,0,0) -- (\laxis,0,0) node [below] {};
  %\draw [->] (0,0,0) -- (0,\laxis,0) node [right] {};
  %\draw [->] (0,0,0) -- (0,0,\laxis) node [left] {};
  %%% axes ticks
  \pgfmathtruncatemacro{\nticks}{floor(\laxis)-1}
  %%% figure
    \shade[ball color=blue!60!cyan,opacity=0.33] (\ltriangle,0) arc (0:90:\ltriangle) {[x={(0,0,1)}] arc (90:0:\ltriangle)} {[y={(0,0,1)}] arc (90:0:\ltriangle)};
\node (pointA) at (0, \ltriangle, 0) {};
\node (pointB) at (0,0,\ltriangle) {};
\node (pointC) at (\ltriangle,0,0) {};
\node (centre) at (sqrt(\ltriangle / 3), sqrt(\ltriangle / 3), sqrt(\ltriangle / 3));
\filldraw[black] (pointA) circle (2pt);
\filldraw[black] (pointB) circle (2pt);
\filldraw[black] (pointC) circle (2pt);
\end{tikzpicture}
\end{gathered}
$
